Opening the Black-Box: A Systematic Review on Explainable AI in Remote Sensing

In recent years, black-box machine learning approaches have become a dominant modeling paradigm for knowledge extraction in remote sensing. Despite the potential benefits of uncovering the inner workings of these models with explainable AI, a comprehensive overview summarizing the explainable AI methods used and their objectives, findings, and challenges in remote sensing applications is still missing. In this paper, we address this gap by performing a systematic review to identify the key trends in the field and shed light on novel explainable AI approaches and emerging directions that tackle specific remote sensing challenges. We also reveal the common patterns of explanation interpretation, discuss the extracted scientific insights, and reflect on the approaches used for the evaluation of explainable AI methods. As such, our review provides a complete summary of the state-of-the-art of explainable AI in remote sensing. Further, we give a detailed outlook on the challenges and promising research directions, representing a basis for novel methodological development and a useful starting point for new researchers in the field.

==> tables/query_ieee.tex <==
("Abstract":earth observation OR "Abstract":remote sensing OR "Abstract":earth science OR "Abstract":satellite data OR "Abstract":satellite image OR "Abstract":aerial image OR "Abstract":aerial data OR "Abstract":airborne image OR "Abstract":airborne data OR "Abstract":radar image OR "Abstract":radar data OR "Abstract":spaceborne image OR "Abstract":spaceborne data OR "Abstract":LiDAR OR "Abstract":SAR OR "Abstract":UAV OR "Abstract":Sentinel OR "Abstract":Landsat OR "Abstract":MODIS OR "Abstract":gaofen OR "Abstract":ceres) AND ("Abstract":"xai" OR "Abstract":"interpret* model" OR "Abstract":"interpret* deep learning" OR "Abstract":"interpret* machine learning" OR "Abstract":"interpret* artificial intelligence" OR "Abstract":"interpret* dl" OR "Abstract":"interpret* ml")
("Abstract":earth observation OR "Abstract":remote sensing OR "Abstract":earth science OR "Abstract":satellite data OR "Abstract":satellite image OR "Abstract":aerial image OR "Abstract":aerial data OR "Abstract":airborne image OR "Abstract":airborne data OR "Abstract":radar image OR "Abstract":radar data OR "Abstract":spaceborne image OR "Abstract":spaceborne data OR "Abstract":LiDAR OR "Abstract":SAR OR "Abstract":UAV OR "Abstract":Sentinel OR "Abstract":Landsat OR "Abstract":MODIS OR "Abstract":gaofen OR "Abstract":ceres) AND ("Abstract":"interpret* AI" OR "Abstract":"explain* model" OR "Abstract":"explain* deep learning" OR "Abstract":"explain* machine learning" OR "Abstract":"explain* artificial intelligence" OR "Abstract":"explain* dl" OR "Abstract":"explain* ml" OR "Abstract":"explain* AI")

("Index Terms":earth observation OR "Index Terms":remote sensing OR "Index Terms":earth science OR "Index Terms":satellite data OR "Index Terms":satellite image OR "Index Terms":aerial image OR "Index Terms":aerial data OR "Index Terms":airborne image OR "Index Terms":airborne data OR "Index Terms":radar image OR "Index Terms":radar data OR "Index Terms":spaceborne image OR "Index Terms":spaceborne data OR "Index Terms":LiDAR OR "Index Terms":SAR OR "Index Terms":UAV OR "Index Terms":Sentinel OR "Index Terms":Landsat OR "Index Terms":MODIS OR "Index Terms":gaofen OR "Index Terms":ceres) AND ("Index Terms":"xai" OR "Index Terms":"interpret* model" OR "Index Terms":"interpret* deep learning" OR "Index Terms":"interpret* machine learning" OR "Index Terms":"interpret* artificial intelligence" OR "Index Terms":"interpret* dl" OR "Index Terms":"interpret* ml")
("Index Terms":earth observation OR "Index Terms":remote sensing OR "Index Terms":earth science OR "Index Terms":satellite data OR "Index Terms":satellite image OR "Index Terms":aerial image OR "Index Terms":aerial data OR "Index Terms":airborne image OR "Index Terms":airborne data OR "Index Terms":radar image OR "Index Terms":radar data OR "Index Terms":spaceborne image OR "Index Terms":spaceborne data OR "Index Terms":LiDAR OR "Index Terms":SAR OR "Index Terms":UAV OR "Index Terms":Sentinel OR "Index Terms":Landsat OR "Index Terms":MODIS OR "Index Terms":gaofen OR "Index Terms":ceres) AND ("Index Terms":"interpret* AI" OR "Index Terms":"explain* model" OR "Index Terms":"explain* deep learning" OR "Index Terms":"explain* machine learning" OR "Index Terms":"explain* artificial intelligence" OR "Index Terms":"explain* dl" OR "Index Terms":"explain* ml" OR "Index Terms":"explain* AI")

("Document Title":earth observation OR "Document Title":remote sensing OR "Document Title":earth science OR "Document Title":satellite data OR "Document Title":satellite image OR "Document Title":aerial image OR "Document Title":aerial data OR "Document Title":airborne image OR "Document Title":airborne data OR "Document Title":radar image OR "Document Title":radar data OR "Document Title":spaceborne image OR "Document Title":spaceborne data OR "Document Title":LiDAR OR "Document Title":SAR OR "Document Title":UAV OR "Document Title":Sentinel OR "Document Title":Landsat OR "Document Title":MODIS OR "Document Title":gaofen OR "Document Title":ceres) AND ("Document Title":"xai" OR "Document Title":"interpret* model" OR "Document Title":"interpret* deep learning" OR "Document Title":"interpret* machine learning" OR "Document Title":"interpret* artificial intelligence" OR "Document Title":"interpret* dl" OR "Document Title":"interpret* ml")
("Document Title":earth observation OR "Document Title":remote sensing OR "Document Title":earth science OR "Document Title":satellite data OR "Document Title":satellite image OR "Document Title":aerial image OR "Document Title":aerial data OR "Document Title":airborne image OR "Document Title":airborne data OR "Document Title":radar image OR "Document Title":radar data OR "Document Title":spaceborne image OR "Document Title":spaceborne data OR "Document Title":LiDAR OR "Document Title":SAR OR "Document Title":UAV OR "Document Title":Sentinel OR "Document Title":Landsat OR "Document Title":MODIS OR "Document Title":gaofen OR "Document Title":ceres) AND ("Document Title":"interpret* AI" OR "Document Title":"explain* model" OR "Document Title":"explain* deep learning" OR "Document Title":"explain* machine learning" OR "Document Title":"explain* artificial intelligence" OR "Document Title":"explain* dl" OR "Document Title":"explain* ml" OR "Document Title":"explain* AI")


==> tables/query_scopus.tex <==
TITLE-ABS-KEY((earth observation) OR (remote sensing) OR (earth science) OR (satellite data) OR (satellite image) OR (aerial image) OR (aerial data) OR (airborne image) OR (airborne data) OR (radar image) OR (radar data) OR (spaceborne image) OR (spaceborne data) OR (LiDAR) OR (SAR) OR (UAV) OR (Sentinel) OR (Landsat) OR (MODIS) OR (gaofen) OR (ceres)) AND TITLE-ABS-KEY("xai" OR "interpret* model" OR "interpret* deep learning" OR "interpret* machine learning" OR "interpret* artificial intelligence" OR "interpret* dl" OR "interpret* ml" OR "interpret* AI" OR "explain* model" OR "explain* deep learning" OR "explain* machine learning" OR "explain* artificial intelligence" OR "explain* dl" OR "explain* ml" OR "explain* AI") AND ( PUBYEAR > 2016 ) AND ( LIMIT-TO ( LANGUAGE,"English" ) )


==> tables/query_springer.tex <==
(earth observation OR remote sensing OR earth science OR satellite data OR satellite image OR aerial image OR aerial data OR airborne image OR airborne data OR radar image OR radar data OR spaceborne image OR spaceborne data OR LiDAR OR SAR OR UAV OR Sentinel OR Landsat OR MODIS OR gaofen OR ceres) AND ("xai" OR "interpret* model" OR "interpret* deep learning" OR "interpret* machine learning" OR "interpret* artificial intelligence" OR "interpret* dl" OR "interpret* ml" OR "interpret* AI" OR "explain* model" OR "explain* deep learning" OR "explain* machine learning" OR "explain* artificial intelligence" OR "explain* dl" OR "explain* ml" OR "explain* AI")


==> tables/summary_table_rows_old.tex <==
Agricultural Monitoring & Backpropagation & \cite{geInterpretableDeep2023} PWGrad-CAM\textsuperscript{\dag Grad-CAM} & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{wolaninEstimatingUnderstanding2020} RAM & CNN &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space & \cite{russwurmSelfattentionRaw2020} Gradient, Attention, Activation Assessment & Transformer, CNN, ConvLSTM, LSTM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space, Feature Selection & \cite{xuInterpretingMultitemporal2021} MDI, Gradient, Attention, Activation Assessment & RF, Transformer, aLSTM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Joint Training & \cite{arunLearningPhysically2022} Explanation Association, LRP & GAN &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation & \cite{mateo-sanchisInterpretableLongShort2023} SHAP, IG & LSTM &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{paudelInterpretabilityDeep2023} SHAP, IG & LSTM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Embedding Space & \cite{saintefaregarnotSatelliteImage2020} Attention & Transformer &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Feature Selection & \cite{orynbaikyzyCropType2020} MDI, GFFS & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design & \cite{celikExplainableArtificial2023} EBM & EBM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design, Perturbation & \cite{martinez-ferrerCropYield2021} GP, Occlusion & GP &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{nayakInterpretableMachine2022} GLM, PFI, ALE, PDP & GLM, RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Joint Training & \cite{rosaLearningCrop2023} Prototype & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{bromsCombinedAnalysis2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{hanExplainableXGBoost2022} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{huberExtremeGradient2022} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{iatrouRepresentationLearning2022} SHAP & RF &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{jonesIdentifyingCauses2022} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{singhSimulationMultispectral2023} SHAP & GLM, SVM, FNN, RF, kNN, GB &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Model Translation, Feature Selection & \cite{newmanExplainableMachine2021} MDI, Rule Extraction & RF, DT &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{brenningSpatialMachinelearning2023} Spatial Variable Importance Profiles\textsuperscript{\dag PFI} & LDA, kNN LDA, RF &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{filippiIdentifyingCrop2022} PFI & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{mateo-sanchisLearningMain2021}  & GP &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation, Embedding Space & \cite{campos-tabernerUnderstandingDeep2020} Occlusion, Activation Assessment & LSTM &  & \ding{51} &  &  &  &  & \ding{51} \\
 &  & \cite{obadicExploringSelfAttention2022} Occlusion, Attention & Transformer &  &  & \ding{51} & \ding{51} &  &  &  \\ \hline 
Atmosphere Monitoring & Backpropagation & \cite{luoExplainableSpatial2022} IG & NN Ensemble &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation, Perturbation & \cite{valdesExplainableAI2022} SHAP, XRAI, Occlusion & CNN &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Embedding Space & \cite{yanNewInterpretable2020} Activation Assessment & FNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{yanUnderstandingGlobal2021} Attention & FNN &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Embedding Space, Joint Training, Feature Selection & \cite{yanSpatialTemporalInterpretable2021} Model Association, MDI, Activation Assessment & RF, NN+ML Ensemble, FNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Feature Selection & \cite{chenEstimationAtmospheric2022} MDI & Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{chenEstimationNearsurface2023} MDI & Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{chenExploringHighresolution2023} MDI & Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design & \cite{maranzanoAdaptiveLASSO2023} GLM\textsuperscript{\dag GLM} & GLM &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Local Approximation & \cite{ebrahimi-khusfiDeterminingContribution2021} SHAP & FNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{shaoEstimationDaily2023} SHAP & GLM, GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{wangEstimatingParticulate2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zipfelMachinelearningBased2022} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation, Feature Selection & \cite{milaEstimatingDaily2023} MDI, SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{liangIntegratingLowcost2023} PFI & aCNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zhenEvaluationMACC2023} PFI, ALE & RF &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\ \cline{2-11}
 & Perturbation, Feature Selection & \cite{wuEstimateNearsurface2023} MDI, PDP & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{valdesMachineLearning2021} SHAP, LIME, Ceteris Paribus Profiles, PFI & RF &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{zhangDataaugmentationApproach2022} SHAP, PDP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Building Mapping & Backpropagation & \cite{chengUncertaintyawareConvolutional2022} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{hasanpourzaryabiUnboxingBlack2022} A*G, DeepLift & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{seydiBDDNetBuilding2023} Grad-CAM & CoAtNet &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{suWhichCAM2022} CAM, Score-CAM, Grad-CAM++, SmoothGrad-CAM++, Grad-CAM & CNN &  &  & \ding{51} & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space & \cite{seydiLeveragingInvolution2023} Attention, Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space, Perturbation & \cite{xiongDisentangledLatent2022} IG, Occlusion, Activation Assessment & Transformer, CNN &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\ \cline{2-11}
 & Local Approximation & \cite{liExplainableDimensionality2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation, Feature Selection & \cite{matinEarthquakeinducedBuildingdamage2021} MDI, SHAP & RF, FNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \hline 
Ecosystem Interactions & Interpretable by Design & \cite{zhouRelativeImportance2021} GAM & GAM &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Interpretable by Design, Local Approximation & \cite{zhuInvestigatingImpacts2022} GLM, SHAP & GLM, GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{descalsLocalInterpretation2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liExploringIndividualized2022} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{zhuExplainableMachine2023} SHAP, PFI & GB &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Human Environment Interaction & Backpropagation & \cite{abitbolInterpretableSocioeconomic2020} GuidedGrad-CAM & CNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{keysMachinelearningApproach2021} LRP & CNN &  & \ding{51} &  & \ding{51} &  &  & \ding{51} \\ \cline{2-11}
 & Backpropagation, Embedding Space, Perturbation & \cite{kucklickTacklingAccuracyinterpretability2023} Occlusion, Grad-CAM, Activation Assessment & GLM, NN Ensemble &  &  & \ding{51} &  &  &  & \ding{51} \\ \cline{2-11}
 & Interpretable by Design & \cite{scepanovicJaneJacobs2021} GLM & GLM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Joint Training & \cite{leveringPredictingLiveability2023} Explanation Association & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{leveringRelationLandscape2021} Explanation Association & CNN &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{chenMeasuringImpacts2020} SHAP & RF &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{dingResidentialGreenness2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{kimModelingPredicting2022} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{scepanovicMedSatPublic2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{temenosNovelInsights2022} SHAP, LIME & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{wangUnpackingInter2023} ALE & RF &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{wojcikPredictingIntraurban2022} PFI & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation, Embedding Space & \cite{stombergExploringWilderness2022} Occlusion, Activation Assessment & CNN &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{prasadEnhancedJoint2023} SHAP, LIME, Occlusion & FNN &  & \ding{51} &  &  &  &  &  \\ \hline 
Hydrology Monitoring & Backpropagation & \cite{blixGaussianProcess2017} Gradient & GP & \ding{51} & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{blixLearningRelevant2022} Gradient & GP &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{chenTransparentDeep2023} Grad-CAM & CNN &  & \ding{51} & \ding{51} & \ding{51} & \ding{51} &  &  \\
 &  & \cite{hongMonitoringVertical2021} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liuExplainableDeep2023} Gradient & CNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{rampalInterpretableDeep2022} Grad-CAM & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation & \cite{yilmazMarineMucilage2023} SHAP, IG & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Perturbation & \cite{jingInterpretingRunoff2023} PDP, IG, DeepLift, Expected Gradients & LSTM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Embedding Space & \cite{pyoCyanobacteriaCell2021} Attention & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zhangFeatureImportance2023} smlp\textsuperscript{\dag Attention} & FNN & \ding{51} & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Interpretable by Design, Local Approximation, Perturbation & \cite{chengImprovedUnderstanding2022} Cubist, ALE, LIME, PFI & Cubist, GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{huWaterStorage2023} SHAP & FNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{saeidiWaterDepth2023} SHAP & RF, GB, DT &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Landcover Mapping & Backpropagation & \cite{deluciaExplainableAI2022} 3DGrad-CAM\textsuperscript{\dag Grad-CAM} & CNN &  & \ding{51} & \ding{51} & \ding{51} & \ding{51} &  &  \\
 &  & \cite{gawlikowskiExplainingEffects2022} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{guoVisualExplanations2023} CSG-CAM\textsuperscript{\dag Grad-CAM}, Score-CAM, Grad-CAM++, Grad-CAM & CNN &  & \ding{51} & \ding{51} &  & \ding{51} &  &  \\
 &  & \cite{huangBetterVisual2022} ERC-CAM\textsuperscript{\dag CAM} & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{hungIntegratingImage2021} XRAI & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{jeonRecursiveVisual2023} Grad-CAM & CNN &  & \ding{51} & \ding{51} &  & \ding{51} &  &  \\
 &  & \cite{Sen2020} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{songMedianpoolingGradCAM2021} MPGrad-CAM\textsuperscript{\dag Grad-CAM}, Grad-CAM++, SmoothGrad-CAM++, Grad-CAM & CNN &  & \ding{51} & \ding{51} &  & \ding{51} &  &  \\
 &  & \cite{vasuResiliencePlasticity2020} CAM & CNN &  & \ding{51} & \ding{51} & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space & \cite{kimFederatedOnboardground2022} CAM, Attention, Grad-CAM, Layer-CAM, Attention, Attention & CNN &  &  & \ding{51} &  & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation, Perturbation & \cite{kakogeorgiouEvaluatingExplainable2021} IG, DeepLift, Gradient, GuidedBackprop, LIME, GuidedGrad-CAM, Grad-CAM, I*G, Occlusion & CNN &  & \ding{51} & \ding{51} & \ding{51} &  &  &  \\ \cline{2-11}
 & Counterfactuals & \cite{dantasCounterfactualExplanations2023} GAN & CNN &  &  & \ding{51} & \ding{51} &  &  &  \\ \cline{2-11}
 & Embedding Space & \cite{chengPolSARImage2021} Activation Assessment & CNN, CapsuleNet &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{guidiciOneDimensionalConvolutional2017} Activation Assessment & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{iencoWeaklySupervised2020} Attention & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{megerExplainingDeep2022} Attention, Activation Assessment & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Embedding Space, Local Approximation & \cite{andersonFuzzyChoquet2018} SHAP, Activation Assessment & NN Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{hungRemoteSensing2020} LIME, Activation Assessment & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{islamEnablingExplainable2020} SHAP, Activation Assessment & NN Ensemble &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\
 &  & \cite{murrayInformationFusion2text2020} SHAP, Activation Assessment & NN Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Example-based & \cite{ishikawaExamplebasedExplainable2023} WIK & CNN &  & \ding{51} &  & \ding{51} & \ding{51} &  & \ding{51} \\ \cline{2-11}
 & Interpretable by Design & \cite{fengBidirectionalFlow2022} Rules & NN+Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{karmakarFrameworkInteractive2022} LDA & LDA &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design, Embedding Space & \cite{huangPhysicallyExplainable2022} LDA, Activation Assessment & NN Ensemble &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Joint Training & \cite{maMulticropFusion2022} Prototype & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Local Approximation & \cite{burguenoScalableApproach2023} SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{elliottIdentifyingCritical2022} SHAP, LIME & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{hosseinyUrbanLand2022} SHAP & SVM, RF, GB, CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{temenosInterpretableDeep2023} SHAP & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{vermaExplainableCustom2021} LIME & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation, Feature Selection & \cite{fisherUncertaintyawareInterpretable2022} MDI, SHAP & RF, CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{jayasingheCausesTea2023} MDI, LIME & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{brenningInterpretingMachinelearning2023} SHAP, ALE, PDP, PFI & RF &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation, Feature Selection & \cite{chenEnhancingLand2023} MDI, SHAP, PFI & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Natural Hazard Monitoring & Backpropagation, Embedding Space & \cite{chenAttributionDeep2023} DeepLift, Attention & NN Ensemble &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space, Perturbation & \cite{bekerDeepLearning2023} Occlusion, Grad-CAM, Activation Assessment & CNN &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation, Perturbation & \cite{kondylatosWildfireDanger2022} SHAP, IG, PDP & LSTM &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Embedding Space, Local Approximation & \cite{fangNewApproach2023} SHAP, Activation Assessment & GAMI-Net &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design & \cite{maxwellExplainableBoosting2021} EBM & EBM &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{stroppianaFullyAutomatic2021} Fuzzy Rules & Rules &  & \ding{51} &  & \ding{51} &  &  & \ding{51} \\
 &  & \cite{youssefLandslideSusceptibility2022} SNN\textsuperscript{\dag FNN} & GAM &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Joint Training & \cite{zhangInterpretableDeep2022} Prototype & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Local Approximation & \cite{abdollahiExplainableArtificial2023} SHAP & FNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{al-najjarNovelMethod2022} SHAP & SVM, RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{aydinPredictingAnalyzing2022} SHAP & RF, GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{dahalExplainableArtificial2022} SHAP & FNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{ibanSnowAvalanche2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{inanExplainableAI2023} SHAP & GB &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{jenaExplainableArtificial2023} SHAP & NN+Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liuResidualNeural2023} SHAP & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{sainiE2AlertNetExplainable2023} SHAP, LIME & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{vegaLandslideModeling2023} SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zhangInsightsGeospatial2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{Taylor2020} PFI, PDP & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation, Feature Selection & \cite{rubiPerformanceComparison2023} MDI, PFI & GLM, SVM, FNN, RF, kNN, GLM, Tree Ensemble, NB &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{alqadhiIntegratedDeep2023} SHAP, PDP, PFI & CNN, NN Ensemble, FNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{chenTunnelGeothermal2023} LIME, Occlusion, PDP & Tree Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{cilliExplainableArtificial2022} SHAP, PFI & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{sunAssessmentLandslide2023} LIME, PDP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{wangXGBoostSHAPApproach2023} SHAP, PDP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Soil Monitoring & Backpropagation, Perturbation & \cite{huangInterpretingConvLSTM2023} SquareGrad, VarGrad, Gradient, PFI, SmoothGrad, I*G, IG & ConvLSTM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{mukhamedievSoilSalinity2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{pradhanNewMethod2022} SHAP & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zhouIdentificationSoil2022} SHAP & SVM &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{Smorkalov2022} PFI & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Surface Temperature Prediction & Backpropagation & \cite{labePredictingSlowdowns2022} LRP & FNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{huPixelLevel2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{kimExaminingRelationship2022} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{luoUnderstandingRelationship2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{shenUsingGeoAI2023} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation, Feature Selection & \cite{milaEstimatingDaily2023} MDI, SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Target Mapping & Backpropagation & \cite{fengSelfMatchingCAM2021} Self-Matching-CAM\textsuperscript{\dag Grad-CAM} & CNN &  &  & \ding{51} &  & \ding{51} &  &  \\
 &  & \cite{liAutomaticBridge2023} CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liDeepNetworks2018} CAM & CNN &  &  &  &  & \ding{51} &  &  \\
 &  & \cite{luoGlassboxingDeep2021} IG, Score-CAM & NN Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{yinG2GradCAMRLObject2023} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space & \cite{liSARBagNetAntehoc2022} CAM, Activation Assessment & BagNet &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Embedding Space, Perturbation & \cite{xiongInterpretableFusion2022} Attention, Empirical Receptive Field, Grad-CAM, Activation Assessment & CNN &  & \ding{51} &  & \ding{51} & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation & \cite{pengClutterinvariantRegularization2023} GuidedBackprop, SHAP & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{zhuLIMEBasedData2022} CAM, LIME & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Embedding Space & \cite{fengPANPart2023} Attention & CNN &  &  &  &  & \ding{51} &  &  \\
 &  & \cite{guoSARAutomatic2021} Activation Assessment & VAE &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liSARADBagNetInterpretable2022} Activation Assessment & BagNet &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{zhouLocalAttention2020} Attention & aCNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{kawauchiSHAPBasedInterpretable2022} SHAP & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\
 &  & \cite{mandeepDeepLearningbased2020} LIME & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{oveisLIMEAssistedAutomatic2023} LIME & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Perturbation & \cite{fengSARTarget2021} Occlusion & NN Ensemble &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Vegetation Monitoring & Backpropagation & \cite{marvasti-zadehCrownCAMInterpretable2023} Eigen-CAM, AugScore-CAM, Crown-CAM\textsuperscript{\dag Grad-CAM}, Score-CAM & CNN &  &  & \ding{51} &  & \ding{51} &  &  \\
 &  & \cite{onishiExplainableIdentification2021} GuidedGrad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Backpropagation, Local Approximation & \cite{jiaStudyingExploiting2021} Deconvolution, Gradient, SHAP, GuidedGrad-CAM & CNN &  &  & \ding{51} &  & \ding{51} &  &  \\ \cline{2-11}
 & Interpretable by Design & \cite{lambertVegetationChange2020} GLM & GLM &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{leon-garzaBigBangbig2020} Fuzzy Rules & FLS &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Joint Training & \cite{nguyenMappingForest2022} Explanation Association & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{abdollahiUrbanVegetation2021} SHAP & FNN &  &  & \ding{51} & \ding{51} & \ding{51} &  &  \\
 &  & \cite{andresiniSILVIAEXplainable2023} SHAP & SVM, RF, GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{arrogante-funesAssessmentRegeneration2023} SHAP & Extra Tree &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{liWidespreadIncreasing2022} SHAP & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Local Approximation, Feature Selection & \cite{sotomayorSupervisedMachine2023} MDI, LIME & GB &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Model Translation & \cite{zhaoBetterUnderstanding2023} Rule Extraction & RF &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{zhaoIdentifyingMangroves2023} Rule Extraction & RF &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Perturbation & \cite{schillerHigherCrop2023} PFI, PDP & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{biassInsightsVulnerability2022} SHAP, PFI & GB &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{mullerFeaturesPredisposing2022} SHAP, PFI & RF &  & \ding{51} &  &  &  &  &  \\ \hline 
Weather Climate Prediction & Backpropagation & \cite{hilburnDevelopmentInterpretation2020} LRP & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{martinUsingSimple2022} LRP & FNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{mayerSubseasonalForecasts2021} LRP & FNN &  & \ding{51} &  &  &  &  &  \\
 &  & \cite{rampalHighresolutionDownscaling2022} Grad-CAM & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{yangPredictorSelection2023} GuidedBackprop & CNN &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Backpropagation, Feature Selection & \cite{liAdvancingSatellite2021} MDI, Grad-CAM & RF, CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Feature Selection & \cite{upadhyayaClassifyingPrecipitation2021} TreeInterpreter & RF &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Joint Training & \cite{barnesThisLooks2022} Prototype\textsuperscript{\dag ProtoPNet} & CNN & \ding{51} & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Local Approximation & \cite{mardianUnderstandingDrivers2023} SHAP & GB &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{silvaUsingExplainable2022} SHAP & GB &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Perturbation, Local Approximation & \cite{antoniadouComparisonDatadriven2023} SHAP, PFI & GLM, RF, SVM, FNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \hline 
Other & Backpropagation & \cite{maddyMIIDAPSAIExplainable2021} Gradient & FNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Feature Selection & \cite{mudeleModelingTemporal2020} MDI & RF &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Interpretable by Design & \cite{karmakarFeaturefreeExplainable2021} LDA & LDA &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Interpretable by Design, Embedding Space & \cite{huangPhysicallyExplainable2022} LDA, Activation Assessment & NN Ensemble &  & \ding{51} &  &  & \ding{51} &  &  \\ \cline{2-11}
 & Joint Training & \cite{bergamascoEXPLAINABLECONVOLUTIONAL2020} Explanation Association & CNN &  & \ding{51} &  & \ding{51} &  &  &  \\ \cline{2-11}
 & Local Approximation & \cite{kimTrueGlobal2023} SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{leeInterpretableMachine2022} SHAP & RF &  & \ding{51} &  & \ding{51} &  &  &  \\
 &  & \cite{wagnerUsingExplainable2022} SHAP & GB &  & \ding{51} &  &  &  &  &  \\ \cline{2-11}
 & Perturbation & \cite{taconetDatadrivenInterpretable2021} PFI, PDP & RF &  & \ding{51} &  &  &  &  &  


==> text/99_search_queries.tex <==
\subsection{Search queries}
\lstset{breakindent=0pt}
\label{apx:search_queries}
Due to the implementation of the search in the databases, they cannot handle deep and nested search queries. For this reason, we repeated different versions of different words, like AI in "explain* AI" and "interpret* AI".

\subsubsection{IEEE}
In the IEEE search, abstract, title, and keywords have the search terms "Abstract", "Document Title", and "Index Terms", respectively. Unfortunately, it is not possible to search with more than 8 wildcards ("*") in one search query. Hence, we split the queries into different parts and merge the results in a second step. The search query cannot include the year or the language, so the results were filtered in the masks of their website.
\lstinputlisting[language = LanQuery,mathescape=true]{tables/query_ieee}

\subsubsection{Scopus}
Scopus has the most powerful search engine for its database. Therefore, it was possible to specify the year of the publication and the language directly in the search query. The search term for abstract, title, and keywords is "TITLE-ABS-KEY".
\lstinputlisting[language = LanQuery,mathescape=true]{tables/query_scopus}

\subsubsection{Springer}
The Springer link search could not be done only on abstract, title, and keywords. Hence, a full-text search was done. The search query cannot include the year or the language, so the results were filtered in the masks of their website.
\lstinputlisting[language = LanQuery,mathescape=true]{tables/query_springer}

\subsubsection{Search query, ML in EO}
This search query was executed in all databases for comparison purposes, its results are shown in Figure \ref{fig:nr_pubs}.
\begin{lstlisting}[language = LanQuery,mathescape=true]
$\Bigl[$earth observation OR remote sensing OR earth science OR $\bigl($(satellite OR aerial OR airborne OR spaceborne OR radar) AND (image OR data)$\bigl)$ OR LiDAR OR SAR OR UAV OR Sentinel OR Landsat OR MODIS OR gaofen OR ceres$\Bigl]$
                        AND
$\Bigl[$deep learning OR machine learning OR artificial intelligence OR dl OR ml OR ai$\Bigl]$
\end{lstlisting}
